Ice sliding games

This paper deals with sliding games, which are a variant of the better known pushpush game. On a given structure (grid, torus...), a robot can move in a specific set of directions, and stops when it hits a block or boundary of the structure. The objective is to place the minimum number of blocks such that the robot can visit all the possible positions of the structure. In particular, we give the exact value of this number when playing on a rectangular grid and a torus. Other variants of this game are also considered, by constraining the robot to stop on each case, or by replacing blocks by walls.

==> carre-pattern-scheme.tex <==

%% image en tikz que tu peux insérer dans une environment figure 
\begin{board}{0}{0}
 
%col et ligne a enlever
%\draw[fill=black!15] (0,6) rectangle (10,9);


\draw[motif] (0,0) rectangle node[fill=white] {$P_n$} (8,10);

\foreach \i in {0,1,...,3}{
  \draw[help lines,dashed] (-0.5,\i) -- (0,\i);
   \draw[help lines,dashed] (8,\i) -- (8.5,\i);
 }
\foreach \i in {7,8,...,10}{
  \draw[help lines,dashed] (-0.5,\i) -- (0,\i);
   \draw[help lines,dashed] (8,\i) -- (8.5,\i);
 }



\mvt{}{-0.5}{1}{2}{1}{east}
\mvt{}{-0.5}{10}{2}{10}{east}
\mvt{}{9.5}{2}{7}{2}{west}
\mvt{}{9.5}{9}{7}{9}{west}

\mvt{}{1}{9}{-0.5}{9}{west}
\mvt{}{8}{1}{9.5}{1}{east}
\mvt{}{8}{10}{9.5}{10}{east}
\mvt{}{1}{2}{-0.5}{2}{west}



%block robot
 \robot{}{-0.5}{1}
 \robot{}{-0.5}{10}
 \robot{}{9.5}{2}
 \robot{}{9.5}{9}

%déplacements

\end{board}

